DeepFD: Automated Fault Diagnosis and Localization for Deep Learning Programs

As Deep Learning (DL) systems are widely deployed for mission-critical applications, debugging such systems becomes essential. Most existing works identify and repair suspicious neurons on the trained Deep Neural Network (DNN), which, unfortunately, might be a detour. Specifically, several existing studies have reported that many unsatisfactory behaviors are actually originated from the faults residing in DL programs. Besides, locating faulty neurons is not actionable for developers, while locating the faulty statements in DL programs can provide developers with more useful information for debugging. Though a few recent studies were proposed to pinpoint the faulty statements in DL programs or the training settings (e.g. too large learning rate), they were mainly designed based on predefined rules, leading to many false alarms or false negatives, especially when the faults are beyond their capabilities. In view of these limitations, in this paper, we proposed DeepFD, a learning-based fault diagnosis and localization framework which maps the fault localization task to a learning problem. In particular, it infers the suspicious fault types via monitoring the runtime features extracted during DNN model training and then locates the diagnosed faults in DL programs. It overcomes the limitations by identifying the root causes of faults in DL programs instead of neurons and diagnosing the faults by a learning approach instead of a set of hard-coded rules. The evaluation exhibits the potential of DeepFD. It correctly diagnoses 52% faulty DL programs, compared with around half (27%) achieved by the best state-of-the-art works. Besides, for fault localization, DeepFD also outperforms the existing works, correctly locating 42% faulty programs, which almost doubles the best result (23%) achieved by the existing works.

==> 2-Background.tex <==
\section{Background}\label{sec:background}
\subsection{Deep Learning Paradigm}
% mention: Deep Learning Training Process (mention weight, loss, activation function, optimizer)

% \victor{where is the figure in page 1 that shows the relation between DNN model and program? 
% I think here we can use it here and highlight the difference between them.
% The current version seems only introduce the DNN model but forget the effects of the program.
% }\bella{update in Introduction, please see if it is fine.}
Deep learning is a stochastic computational paradigm that makes prediction through hierarchical layers of \textit{neurons} that are inter-dependent to form a deep neural network (DNN). 
% Each neuron performs computation by applying a non-linear \textit{activation function} to the weighted sum of the neuron's inputs. Before making prediction, a DNN is trained using appropriate \textit{loss functions} and \textit{optimizers}~\cite{goodfellow2016deep} on the computation results of the neurons.

\begin{comment}
Each neuron can be viewed as a processing unit that accepts the inputs from its preceding layer, aggregates the \textit{weights} in the connected edges, applies a non-linear \textit{activation function} to the inputs, and passes the resulting value to the connected neurons at the succeeding layer. 
Such forward computational propagation ends at the last layer, i.e., the \textit{output layer}. The resulting output is then compared to the expected output. The difference between the actual output and the expected output is quantified by \textit{loss function}, which is then used to adjust the weights of the neurons during \textit{back propagation} with different \textit{optimizers}~\cite{goodfellow2016deep}. \scc{Other than the first sentence, are other sentences necessary?}
\end{comment}

\subsection{Mutation Testing}
% what is fault seeding in mutation testing. Why it is useful for auto debug and repair tool.
Mutation testing~\cite{offutt2001mutation,mutationSurvey11} is a method of creating variants, called mutants, of a program by mutating a small piece of code in it. The code mutation is also known as fault seeding~\cite{FaultSeeding97,faultSeeding07}. A mutant is said to be killed by a test if its executions on the mutant and on the original program lead to different test outcomes~\cite{mutationSurvey11}.

\begin{comment}
Mutation testing~\cite{offutt2001mutation,mutationSurvey11} is a systematic method of fault seeding~\cite{FaultSeeding97,faultSeeding07}. 
By seeding faults intentionally to an original program $\mathcal{P}$, a set of faulty programs $\mathcal{P}'$s (\textit{mutants}) are generated with respected to $\mathcal{P}$. 
Given a test input, if the behavior of a mutant differs from its original program, the mutant is \textit{killed} by this test input. 
The percentage of the killed mutant (i.e., mutation score) is often used to evaluate the quality of a test suit~\cite{mutationSurvey11}. In general, the availability of a mutation tool that can inject changes imitating real faults is useful in assessing automated testing tools such as debugging or repair tools~\cite{mutationSurvey11}. 
\end{comment}
% In addition, the intuition of the fault seeding is to imitate the real faults made by developers, so the more likely the fault made by developers, the more representative is the seeded fault~\cite{mutationSurvey11}. 
% \victor{I cannot see the connection between this sentence and the others.}\bella{updated.}
% Mutants are based on well-defined mutation operators that either mimic typical programming errors (such as using the wrong operator or variable name) or force the creation of valuable tests (such as dividing each expression by zero). The purpose is to help the tester develop effective tests or locate weaknesses in the test data used for the program or in sections of the code that are seldom or never accessed during execution.
% Mutation testing relies on the assumption that test suites that can kill more mutants
% % achieving a high mutation score
% are more likely to be able to expose the faults that affect the original program.
% This assumption is more likely to hold 
% if the mutation operators being used are based on representative real faults, rather than on arbitrary changes to the program under test~\cite{bugrepair20}.
% so the more representative the seeded fault imitating the real fault, the more useful is the mutation testing.

% The faults seeded are expected to be representative to imitate the real faults that could happen.
% The underlying of fault seeding is to imitate the real faults that could happen in 
% each of which slightly modifies $\mathcal{P}$ according to the seeded fault. 

% while test suites achieving a low mutation score need to be improved. 
% 

% Moreover, availability of a mutation tool that can inject changes imitating real faults is extremely useful in assessing automated testing tools, such as test generators or repair tools.

% % mention: mutation testing. Mutation operator. Kill mutant.
% Fault seeding inserts ``typical'' faults into a system.



\subsection{Faults, Symptoms and Fix Patterns}
There are several empirical studies~\cite{tfbug18,bugcharacter19,taxonomy20,bugrepair20} characterized and categorized the faults, their symptoms and fix patterns in developing deep learning system from different aspects with various granularities. 
To ease the comprehension of these terms, we explain the terms with examples excerpted from the corresponding publication.

\textbf{Faults~\cite{taxonomy20}} (also known as \textit{bugs}~\cite{bugcharacter19,bugrepair20} or \textit{root causes}~\cite{tfbug18}) in DL system are cases when man-made mistakes occur
% \cx{I think a verb is expected to be added here, for instance 'occur'. Or we can reorganize the structure of this sentence.}
during DL development and training. They usually lead to functionally insufficient performance~\cite{taxonomy20}. 
Typical types of faults include wrong data type, inappropriate hyperparameter such as learning rate, unsuitable optimizer, etc. 

\textbf{{Symptoms}~\cite{bugrepair20}} (also known as the \textit{effects}~\cite{tfbug18} or \textit{impact} of faults~\cite{bugcharacter19}) describe the abnormal behaviors of DL systems caused by certain faults~\cite{bugcharacter19,bugrepair20}. 
The most common effects of faults include crash and low efficiency (i.e., the program exhibits extraordinarily poor accuracy, loss, or other unexpected outputs during the training phase)~\cite{tfbug18,bugrepair20}.
% \victor{I think the term ``symptoms'' is more common.}\bella{updated.}

\textbf{Fix patterns~\cite{bugrepair20}} prescribe a bunch of plausible \textbf{patches} that could be potentially fix or mitigate the target symptom. Islam et al.~\cite{bugrepair20} concluded 15 fix patterns including changing the optimization function, changing the loss function, etc. The corresponding patches are instances of certain fix pattern. For example, {changing the activation function from {sigmoid} to {linear} activation function} is an instantiated patch for the fix pattern of \textit{changing the activation function}.

\scc{I am unsure if this Section is necessary. Instead, I expect a section explaining the motivating example and illustrating the limitations of state-of-the-art, challenges, insight and our solutions intuitively. Terminologies should be introduced while explaining the example and our solutions intuitively. The current presentation lacks an interesting story line.}
% For example, changing activation function is a fix pattern which will be studied later.
% \victor{Please see if it is true.}
% A fix patch of this pattern could be that ``changing the \textit{sigmoid} activation function into \textit{linear} activation function.
% \victor{updated, please check.}\bella{updated.}
% A fix patch of this pattern could be that ``changing the \textit{sigmoid} activations into \textit{linear} activations out the speech recognition, it gave me a gain''~\cite{taxonomy20}.
% \victor{This example is a fix, or a fix pattern?}
% In this paper, we regard a patch is effective is it brings a gain in accuracy or a decrease in loss.
% \victor{any threshold?}\bella{No.}
% In this paper, we focused on faults which result in low effectiveness, because 

% The existing works have summarized the fault types with different granularities~\cite{tfbug18,bugcharacter19,taxonomy20}, characterized and their symptoms~\cite{tfbug18,bugcharacter19} and fix patterns~\cite{bugrepair20}. 

% % mention: Fault, root causes, symptoms, fix patterns
% Zhang et al.~\cite{tfbug18} concluded seven types of fault
% A real fault in DL systems is a case when a human-made mistake during the development or training of a DL component, leads to functionally insufficient performance~\cite{taxonomy20}.

% Zhang et al.~\cite{tfbug18} concluded four symptoms: Error (Crash), Low effectiveness, Low efficiency and Unknown. Islam et al.~\cite{bugcharacter19} further elaborated six symptoms: Bad Performance, Crash, Data Corruption (the data is corrupted as it flows through the network, leading to the unexpected output), Hang (software runs for a long period of time without providing the desired output), Incorrect Functionality (the software behaves in an unexpected way without any runtime or compile-time error/warning) and Memory Out of Bound.

% The increasing dependence of safety-critical systems on DL networks makes the types of faults that can occur in such systems a crucial topic. 
% potential severity of fault in these systems has motivated intensive studies to understand and detect the faults in DL systems
% The above-mentioned learning process is implemented in software.

% We consider that a DL fault has taken place when the behaviour of the DL component is inadequate for the task at hand (i.e., it is ``functionally insufficient'', in line with ISO/PAS 21448:2019 [6]) and the root cause for such inadequacy is a human mistake that occurred during DL development and training.

% \subsubsection{\textbf{Fix Patterns in Deep Learning programs}}

% Islam et al.~\cite{bugrepair20} studied 320 posts in Stack Overflow and 347 bug fix codes in GitHub, and concluded 15 fix patterns. 
% In total, we have studied 320 bug fix codes 


% \subsection{Multi-Label Classification}
% Multi-label classification task.



